MIBench: A Comprehensive Framework for Benchmarking Model Inversion Attack and Defense

Model Inversion (MI) attacks aim at leveraging the output information of target models to reconstruct privacy-sensitive training data, raising critical concerns regarding the privacy vulnerabilities of Deep Neural Networks (DNNs). Unfortunately, in tandem with the rapid evolution of MI attacks, the absence of a comprehensive benchmark with standardized metrics and reproducible implementations has emerged as a formidable challenge. This deficiency has hindered objective comparison of methodological advancements and reliable assessment of defense efficacy. To address this critical gap, we build the first practical benchmark named MIBench for systematic evaluation of model inversion attacks and defenses. This benchmark bases on an extensible and reproducible modular-based toolbox which currently integrates a total of 19 state-of-the-art attack and defense methods and encompasses 9 standardized evaluation protocols. Capitalizing on this foundation, we conduct extensive evaluation from multiple perspectives to holistically compare and analyze various methods across different scenarios, such as the impact of target resolution, model predictive power, defense performance and adversarial robustness.

==> tables/celeba_celeba_ir152/base.tex <==
\begin{table}[!ht]
    \setlength{\tabcolsep}{5pt}
    \normalsize
    \centering
    \caption{\todo{table}}
    \label{}
    \begin{threeparttable} 
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccccc}
        \toprule
\textbf{Method} & $\uparrow{\mathbf{Acc}@1}$ & $\uparrow{\mathbf{Acc}@5}$ & $\downarrow\mathbf{\delta}_{eval}$ & $\downarrow\mathbf{\delta}_{face}$ & $\downarrow\textbf{FID}$\\ \midrule
GMI & $0.207\pm0.092$ & $0.381\pm0.145$ & $1875.897\pm202.720$ & $1.153\pm0.152$ & $51.840$\\
KEDMI & $0.640\pm0.008$ & $0.878\pm0.007$ & $1345.591\pm239.542$ & $0.771\pm0.180$ & $34.289$\\
Mirror(white) & $0.043\pm0.004$ & $0.105\pm0.011$ & $2368.171\pm11725.341$ & $1.344\pm0.265$ & $40.444$\\
PPA & $0.231\pm0.070$ & $0.348\pm0.085$ & $1738.922\pm402.082$ & $1.171\pm0.355$ & $33.208$\\
PLGMI & $\mathbf{0.998}\pm0.000$ & $\mathbf{0.999}\pm0.000$ & $\mathbf{892.373}\pm153.043$ & $\mathbf{0.452}\pm0.109$ & $23.360$\\
LOMMA+GMI & $0.698\pm0.096$ & $0.840\pm0.057$ & $1407.781\pm239.174$ & $0.764\pm0.163$ & $45.472$\\
LOMMA+KEDMI & $0.838\pm0.006$ & $0.950\pm0.002$ & $1230.080\pm244.846$ & $0.665\pm0.219$ & $40.472$\\
\bottomrule
    \end{tabular}
    }
    \end{threeparttable}
    % \vspace{-1em}
\end{table}

==> tables/celeba_celeba_ir152/blackbase.tex <==
\begin{table}[!ht]
    \setlength{\tabcolsep}{5pt}
    \normalsize
    \centering
    \caption{\todo{table}}
    \label{}
    \begin{threeparttable} 
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccccc}
        \toprule
\textbf{Method} & $\uparrow{\mathbf{Acc}@1}$ & $\uparrow{\mathbf{Acc}@5}$ & $\downarrow\mathbf{\delta}_{eval}$ & $\downarrow\mathbf{\delta}_{face}$ & $\downarrow\textbf{FID}$\\ \midrule
BREP & $0.452\pm0.012$ & $0.724\pm0.014$ & $1447.611\pm217.962$ & $0.852\pm0.161$ & $49.880$\\
Mirror(black) & $0.116\pm0.009$ & $0.261\pm0.009$ & $24209.293\pm667319.148$ & $1.214\pm0.298$ & $127.812$\\
C2F & $0.020\pm0.002$ & $0.058\pm0.003$ & $7639.523\pm176021.713$ & $1.376\pm0.311$ & $55.991$\\
LOKT & $\mathbf{0.789}\pm0.006$ & $\mathbf{0.937}\pm0.003$ & $\mathbf{1266.716}\pm244.974$ & $\mathbf{0.688}\pm0.160$ & $\mathbf{15.228}$\\
\bottomrule
    \end{tabular}
    }
    \end{threeparttable}
    % \vspace{-1em}
\end{table}

==> tables/celeba_celeba_ir152/blackprdc.tex <==
\begin{table}[!ht]
    \setlength{\tabcolsep}{5pt}
    \normalsize
    \centering
    \caption{\todo{table}}
    \label{}
    \begin{threeparttable} 
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccccc}
        \toprule
\textbf{Method} & $\uparrow\textbf{Precision}$ & $\uparrow\textbf{Recall}$ & $\uparrow\textbf{Density}$ & $\uparrow\textbf{Coverage}$\\ \midrule
BREP & $0.062\pm0.147$ & $0.109\pm0.204$ & $0.021\pm0.034$ & $0.037\pm0.054$\\
Mirror(black) & $0.187\pm0.293$ & $0.016\pm0.082$ & $0.028\pm0.041$ & $0.038\pm0.047$\\
C2F & $0.099\pm0.230$ & $0.033\pm0.137$ & $0.016\pm0.032$ & $0.023\pm0.040$\\
LOKT & $\mathbf{0.351}\pm0.322$ & $0.114\pm0.195$ & $\mathbf{0.134}\pm0.119$ & $\mathbf{0.208}\pm0.155$\\
\bottomrule
    \end{tabular}
    }
    \end{threeparttable}
    % \vspace{-1em}
\end{table}

==> tables/celeba_celeba_ir152/prdc.tex <==
\begin{table}[!ht]
    \setlength{\tabcolsep}{5pt}
    \normalsize
    \centering
    \caption{\todo{table}}
    \label{}
    \begin{threeparttable} 
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccccc}
        \toprule
\textbf{Method} & $\uparrow\textbf{Precision}$ & $\uparrow\textbf{Recall}$ & $\uparrow\textbf{Density}$ & $\uparrow\textbf{Coverage}$\\ \midrule
GMI & $0.178\pm0.204$ & $0.604\pm0.249$ & $0.040\pm0.041$ & $0.092\pm0.087$\\
KEDMI & $0.177\pm0.253$ & $0.032\pm0.110$ & $0.058\pm0.068$ & $0.092\pm0.095$\\
Mirror(white) & $0.125\pm0.207$ & $0.367\pm0.327$ & $0.023\pm0.035$ & $0.049\pm0.067$\\
PPA & $0.141\pm0.213$ & $0.414\pm0.327$ & $0.026\pm0.039$ & $0.058\pm0.077$\\
PLGMI & $0.231\pm0.246$ & $0.396\pm0.264$ & $0.100\pm0.093$ & $0.194\pm0.155$\\
LOMMA+GMI & $0.076\pm0.137$ & $\mathbf{0.671}\pm0.229$ & $0.022\pm0.030$ & $0.054\pm0.067$\\
LOMMA+KEDMI & $0.108\pm0.243$ & $0.000\pm0.001$ & $0.043\pm0.070$ & $0.049\pm0.070$\\
\bottomrule
    \end{tabular}
    }
    \end{threeparttable}
    % \vspace{-1em}
\end{table}

==> tables/defense.tex <==
\begin{table}[!ht]
    \setlength{\tabcolsep}{5pt}
    \normalsize
    \centering
    \caption{Evaluation on multiple MI defense strategies.}
    \label{table:defense}
    \begin{threeparttable} 
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccccccccc}
        \toprule
\multirow{2}{*}{Method} & \multicolumn{5}{c}{$\uparrow$\textbf{Acc}@1} &\multicolumn{5}{c}{$\uparrow$\textbf{Acc}@5} \\
\cmidrule(lr){2-6}\cmidrule(lr){7-11} & ${\mathbf{NO \; Defense}}$ & ${\mathbf{MID}}$ & $\mathbf{BiDO}$ & $\mathbf{LS}$ & $\textbf{TL}$& ${\mathbf{NO Defense}}$ & ${\mathbf{MID}}$ & $\mathbf{BiDO}$ & $\mathbf{LS}$ & $\textbf{TL}$\\ \midrule
GMI & $0.080\pm0.086$ & $0.116\pm0.114$ & $0.102\pm0.050$ & $0.170\pm0.076$ & $\textbf{0.046}\pm0.039$ & $0.088\pm0.059$ & $0.172\pm0.146$ & $0.274\pm0.213$ & $\textbf{0.017}\pm0.014$ & $0.050\pm0.030$\\
KEDMI & $0.504\pm0.017$ & $0.722\pm0.029$ & $0.314\pm0.017$ & $0.398\pm0.026$ & $\textbf{0.210}\pm0.031$ & $0.358\pm0.025$ & $0.548\pm0.030$ & $0.736\pm0.016$ & $\textbf{0.074}\pm0.005$ & $0.118\pm0.024$\\
Mirror & $0.404\pm0.055$ & $0.574\pm0.039$ & $0.394\pm0.017$ & $0.512\pm0.039$ & $\textbf{0.196}\pm0.032$ & $0.350\pm0.052$ & $0.456\pm0.042$ & $0.626\pm0.036$ & $\textbf{0.110}\pm0.027$ & $0.200\pm0.031$\\
PPA & $0.912\pm0.039$ & $0.952\pm0.027$ & $0.798\pm0.066$ & $0.860\pm0.059$ & $\textbf{0.580}\pm0.065$ & $0.756\pm0.077$ & $0.938\pm0.019$ & $0.976\pm0.010$ & $\textbf{0.570}\pm0.059$ & $0.760\pm0.080$\\
PLGMI & $1.000\pm0.000$ & $1.000\pm0.000$ & $0.982\pm0.004$ & $0.990\pm0.000$ & $\textbf{0.894}\pm0.021$ & $0.962\pm0.019$ & $0.996\pm0.004$ & $0.998\pm0.003$ & $\textbf{0.936}\pm0.016$ & $0.978\pm0.010$\\
LOMMA+GMI & $0.367\pm0.169$ & $0.496\pm0.193$ & $0.225\pm0.151$ & $0.322\pm0.186$ & $\textbf{0.166}\pm0.075$ & $0.308\pm0.118$ & $0.381\pm0.182$ & $0.513\pm0.199$ & $\textbf{0.085}\pm0.058$ & $0.169\pm0.096$\\
LOMMA+KEDMI & $0.463\pm0.151$ & $0.586\pm0.186$ & $0.386\pm0.015$ & $0.472\pm0.012$ & $\textbf{0.310}\pm0.013$ & $0.520\pm0.023$ & $0.630\pm0.024$ & $0.729\pm0.005$ & $\textbf{0.079}\pm0.013$ & $0.160\pm0.014$\\

        \bottomrule
    \end{tabular}
    }
    \end{threeparttable}
    % \vspace{-1em}
\end{table}

==> tables/diff_acc/acc.tex <==
\begin{table}[!ht]
    \setlength{\tabcolsep}{5pt}
    \normalsize
    \centering
    \caption{Evaluation on the ResNet-152 with varied predictive power. The \textbf{low} column represents 91.01\% test accuracy for ResNet-152. The \textbf{mid} column demonstrates 95.92\% test accuracy. The \textbf{high} column stands for 98.25\%, which is identical to the ResNet-152 in Table \ref{white:different methods}.}
    \label{table:different acc-acc}
    \begin{threeparttable} 
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccccc}
        \toprule
 \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{$\uparrow$\textbf{Acc}@1} &\multicolumn{3}{c}{$\uparrow$\textbf{Acc}@5} \\
 \cmidrule(lr){2-4}\cmidrule(lr){5-7} & 
 \textbf{low} & \textbf{mid} & \textbf{high} & \textbf{low} & \textbf{mid} & \textbf{high}  \\ \midrule
GMI & $0.175\pm0.015$ & $0.223\pm0.113$ & $0.153\pm0.077$ & $0.308\pm0.023$ & $0.368\pm0.127$ & $0.265\pm0.093$\\
KEDMI & $0.438\pm0.010$ & $0.434\pm0.013$ & $0.468\pm0.015$ & $0.609\pm0.011$ & $0.620\pm0.016$ & $0.664\pm0.011$\\
Mirror(white) & $0.490\pm0.015$ & $0.462\pm0.028$ & $0.311\pm0.014$ & $0.650\pm0.017$ & $0.626\pm0.024$ & $0.509\pm0.021$\\
PPA & $0.723\pm0.038$ & $0.829\pm0.039$ & $0.840\pm0.036$ & $0.840\pm0.031$ & $0.902\pm0.028$ & $0.923\pm0.026$\\
PLGMI & $\mathbf{0.886}\pm0.007$ & $\mathbf{0.965}\pm0.005$ & $\mathbf{0.998}\pm0.002$ & $\mathbf{0.932}\pm0.007$ & $\mathbf{0.981}\pm0.004$ & $\mathbf{0.999}\pm0.001$\\
LOMMA+GMI & $0.484\pm0.122$ & $0.517\pm0.119$ & $0.557\pm0.111$ & $0.645\pm0.111$ & $0.670\pm0.104$ & $0.678\pm0.096$\\
LOMMA+KEDMI & $0.593\pm0.012$ & $0.654\pm0.006$ & $0.711\pm0.007$ & $0.770\pm0.011$ & $0.823\pm0.007$ & $0.860\pm0.006$\\
\bottomrule
    \end{tabular}
    }
    \end{threeparttable}
    % \vspace{-1em}
\end{table}

==> tables/diff_acc/dist.tex <==
\begin{table}[!ht]
    \setlength{\tabcolsep}{5pt}
    \normalsize
    \centering
    \caption{Feature Distance for evaluation on the ResNet-152 with varied predictive power.}
    \label{table:different acc-dist}
    \begin{threeparttable} 
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccccc}
        \toprule
 \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{$\downarrow\mathbf{\delta}_{eval}$ } &\multicolumn{3}{c}{$\downarrow\mathbf{\delta}_{face}$} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7} & \textbf{low} & \textbf{mid} & \textbf{high} & \textbf{low} & \textbf{mid} & \textbf{high}  \\ \midrule
GMI & $2367.287\pm355.743$ & $2374.313\pm310.858$ & $2442.667\pm298.597$ & $1.222\pm0.215$ & $1.130\pm0.191$ & $1.300\pm0.176$\\
KEDMI & $2091.583\pm607.615$ & $2124.271\pm587.946$ & $2005.154\pm510.527$ & $0.941\pm0.371$ & $0.963\pm0.346$ & $0.930\pm0.300$\\
Mirror & $1784.638\pm496.468$ & $1812.977\pm440.571$ & $1979.211\pm427.343$ & $0.898\pm0.312$ & $0.912\pm0.277$ & $0.996\pm0.258$\\
PPA & $1549.006\pm521.791$ & $1413.097\pm468.792$ & $1374.967\pm387.380$ & $0.729\pm0.274$ & $0.683\pm0.240$ & $0.657\pm0.195$\\
PLGMI & $\mathbf{1328.291}\pm499.408$ & $\mathbf{1163.656}\pm362.421$ & $\mathbf{967.295}\pm222.725$ & $\mathbf{0.595}\pm0.214$ & $\mathbf{0.557}\pm0.153$ & $\mathbf{0.486}\pm0.103$\\
LOMMA+GMI & $1973.187\pm427.428$ & $2071.116\pm381.253$ & $1948.976\pm317.310$ & $0.899\pm0.251$ & $0.894\pm0.206$ & $0.949\pm0.221$\\
LOMMA+KEDMI & $1806.098\pm528.101$ & $1771.850\pm504.995$ & $1685.514\pm486.419$ & $0.782\pm0.305$ & $0.734\pm0.272$ & $0.759\pm0.289$\\


\bottomrule
    \end{tabular}
    }
    \end{threeparttable}
    % \vspace{-1em}
\end{table}

==> tables/diff_loss/prdc.tex <==
\begin{table}[!ht]
    \setlength{\tabcolsep}{5pt}
    \normalsize
    \centering
    \caption{\todo{table}}
    \label{}
    \begin{threeparttable} 
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccccc}
        \toprule
\textbf{Loss Function} & $\uparrow\textbf{Precision}$ & $\uparrow\textbf{Recall}$ & $\uparrow\textbf{Density}$ & $\uparrow\textbf{Coverage}$\\ \midrule
CE & $0.244\pm0.238$ & $0.345\pm0.269$ & $0.052\pm0.068$ & $0.100\pm0.097$\\
Poincar\'e & $0.259\pm0.243$ & $0.322\pm0.266$ & $0.060\pm0.075$ & $0.112\pm0.102$\\
Max Margin & $0.260\pm0.253$ & $0.311\pm0.272$ & $0.058\pm0.076$ & $0.107\pm0.108$\\
Logit & $\mathbf{0.267}\pm0.244$ & $0.313\pm0.267$ & $\mathbf{0.062}\pm0.084$ & $\mathbf{0.116}\pm0.109$\\
CE$^+$ & $0.236\pm0.251$ & $0.279\pm0.241$ & $0.053\pm0.066$ & $0.100\pm0.102$\\
Poincar\'e$^+$ & $0.248\pm0.256$ & $\mathbf{0.372}\pm0.280$ & $0.057\pm0.077$ & $0.110\pm0.117$\\
Max Margin$^+$ & $0.260\pm0.264$ & $0.290\pm0.258$ & $0.057\pm0.076$ & $0.106\pm0.111$\\
Logit$^+$ & $0.266\pm0.264$ & $0.266\pm0.262$ & $0.059\pm0.073$ & $0.108\pm0.098$\\
\bottomrule
    \end{tabular}
    }
    \end{threeparttable}
    % \vspace{-1em}
\end{table}


==> tables/ffhq256_celeba224_resnet152/prdc.tex <==
\begin{table}[!ht]
    \setlength{\tabcolsep}{5pt}
    \normalsize
    \centering
    \caption{\todo{table}}
    \label{}
    \begin{threeparttable} 
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccccc}
        \toprule
\textbf{Method} & $\uparrow\textbf{Precision}$ & $\uparrow\textbf{Recall}$ & $\uparrow\textbf{Density}$ & $\uparrow\textbf{Coverage}$\\ \midrule
GMI & $0.029\pm0.082$ & $0.558\pm0.302$ & $0.006\pm0.012$ & $0.014\pm0.027$\\
KEDMI & $0.026\pm0.110$ & $0.023\pm0.108$ & $0.007\pm0.017$ & $0.011\pm0.026$\\
Mirror & $0.271\pm0.261$ & $0.311\pm0.270$ & $0.063\pm0.062$ & $0.124\pm0.110$\\
PPA & $\mathbf{0.332}\pm0.273$ & $0.337\pm0.275$ & $\mathbf{0.088}\pm0.075$ & $\mathbf{0.173}\pm0.129$\\
PLGMI & $0.016\pm0.094$ & $0.000\pm0.000$ & $0.005\pm0.015$ & $0.008\pm0.019$\\
LOMMA+GMI & $0.039\pm0.095$ & $\mathbf{0.629}\pm0.305$ & $0.008\pm0.015$ & $0.020\pm0.035$\\
LOMMA+KEDMI & $0.024\pm0.117$ & $0.009\pm0.066$ & $0.006\pm0.019$ & $0.009\pm0.022$\\
\bottomrule
    \end{tabular}
    }
    \end{threeparttable}
    % \vspace{-1em}
\end{table}

==> tables/ffhq256_facescrub224_resnest101/prdc.tex <==
\begin{table}[!ht]
    \setlength{\tabcolsep}{5pt}
    \normalsize
    \centering
    \caption{\todo{table}}
    \label{}
    \begin{threeparttable} 
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccccc}
        \toprule
\textbf{Method} & $\uparrow\textbf{Precision}$ & $\uparrow\textbf{Recall}$ & $\uparrow\textbf{Density}$ & $\uparrow\textbf{Coverage}$\\ \midrule
GMI & $0.022\pm0.068$ & $0.722\pm0.260$ & $0.004\pm0.010$ & $0.011\pm0.024$\\
KEDMI & $0.023\pm0.091$ & $0.014\pm0.067$ & $0.003\pm0.010$ & $0.006\pm0.018$\\
Mirror & $0.229\pm0.237$ & $0.347\pm0.281$ & $0.049\pm0.070$ & $0.095\pm0.103$\\
PPA & $\mathbf{0.255}\pm0.238$ & $0.320\pm0.264$ & $\mathbf{0.060}\pm0.081$ & $\mathbf{0.113}\pm0.104$\\
PLGMI & $0.030\pm0.122$ & $0.005\pm0.049$ & $0.011\pm0.028$ & $0.016\pm0.036$\\
LOMMA+GMI & $0.016\pm0.063$ & $\mathbf{0.732}\pm0.270$ & $0.003\pm0.008$ & $0.008\pm0.019$\\
LOMMA+KEDMI & $0.030\pm0.132$ & $0.001\pm0.019$ & $0.004\pm0.015$ & $0.005\pm0.017$\\
\bottomrule
    \end{tabular}
    }
    \end{threeparttable}
    % \vspace{-1em}
\end{table}

==> tables/ffhq256_facescrub224_resnet152/blackbase.tex <==
\begin{table}[!ht]
    \setlength{\tabcolsep}{5pt}
    \normalsize
    \centering
    \caption{Comparison between black-box MI attacks on higher resolution scenario.}
    \label{black:high resolution}
    \begin{threeparttable} 
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccccc}
        \toprule
\textbf{Method} & $\uparrow{\mathbf{Acc}@1}$ & $\uparrow{\mathbf{Acc}@5}$ & $\downarrow\mathbf{\delta}_{eval}$ & $\downarrow\mathbf{\delta}_{face}$ & $\downarrow\textbf{FID}$\\ \midrule
BREPMI & $0.342\pm0.013$ & $0.622\pm0.026$ & $134.263\pm31.441$ & $1.067\pm0.208$ & $105.489$\\
Mirror (black) & $\textbf{0.611}\pm0.051$ & $\textbf{0.862}\pm0.018$ & $198.609\pm40.255$ & $\textbf{1.049}\pm0.192$ & $92.413$\\
C2FMI & $0.414\pm0.017$ & $0.686\pm0.018$ & $439.659\pm93.688$ & $1.592\pm0.249$ & $\textbf{47.317}$\\
LOKT & $0.328\pm0.004$ & $0.553\pm0.010$ & $\mathbf{126.964}\pm36.434$ & $1.122\pm0.284$ & $127.709$\\
\bottomrule
    \end{tabular}
    }
    \end{threeparttable}
    % \vspace{-1em}
\end{table}

==> tables/ffhq64_facescrub64_ir152/blackbase.tex <==
\begin{table}[!ht]
    \setlength{\tabcolsep}{5pt}
    \normalsize
    \centering
    \caption{Comparison between black-box MI attacks.}
    \label{black:different methods}
    \begin{threeparttable} 
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccccc}
        \toprule
\textbf{Method} & $\uparrow{\mathbf{Acc}@1}$ & $\uparrow{\mathbf{Acc}@5}$ & $\downarrow\mathbf{\delta}_{eval}$ & $\downarrow\mathbf{\delta}_{face}$ & $\downarrow\textbf{FID}$\\ \midrule
BREPMI & $0.354\pm0.013$ & $0.608\pm0.015$ & $2178.587\pm357.194$ & $0.971\pm0.186$ & $74.519$\\
Mirror(black) & $0.526\pm0.031$ & $0.729\pm0.020$ & $1972.175\pm427.391$ & $0.854\pm0.239$ & $54.231$\\
C2FMI & $0.263\pm0.009$ & $0.459\pm0.016$ & $2061.995\pm534.556$ & $1.011\pm0.265$ & $\textbf{43.488}$\\
LOKT & $\textbf{0.834}\pm0.010$ & $\textbf{0.918}\pm0.013$ & $\textbf{1533.071}\pm402.791$ & $\textbf{0.694}\pm0.169$ & $71.701$\\
\bottomrule
    \end{tabular}
    }
    \end{threeparttable}
    % \vspace{-1em}
\end{table}

==> tables/ffhq64_facescrub64_ir152_low/base.tex <==
\begin{table}[!ht]
    \setlength{\tabcolsep}{5pt}
    \normalsize
    \centering
    \caption{\todo{table}}
    \label{}
    \begin{threeparttable} 
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccccc}
        \toprule
\textbf{Method} & $\uparrow{\mathbf{Acc}@1}$ & $\uparrow{\mathbf{Acc}@5}$ & $\downarrow\mathbf{\delta}_{eval}$ & $\downarrow\mathbf{\delta}_{face}$ & $\downarrow\textbf{FID}$\\ \midrule
GMI & $0.175\pm0.015$ & $0.308\pm0.023$ & $2367.287\pm355.743$ & $1.222\pm0.215$ & $63.446$\\
KEDMI & $0.438\pm0.010$ & $0.609\pm0.011$ & $2091.583\pm607.615$ & $0.941\pm0.371$ & $66.113$\\
Mirror & $0.490\pm0.015$ & $0.650\pm0.017$ & $1784.638\pm496.468$ & $0.898\pm0.312$ & $\mathbf{30.312}$\\
PPA & $0.723\pm0.038$ & $0.840\pm0.031$ & $1549.006\pm521.791$ & $0.729\pm0.274$ & $32.213$\\
PLGMI & $\mathbf{0.886}\pm0.007$ & $\mathbf{0.932}\pm0.007$ & $\mathbf{1328.291}\pm499.408$ & $\mathbf{0.595}\pm0.214$ & $68.022$\\
LOMMA+GMI & $0.484\pm0.122$ & $0.645\pm0.111$ & $1973.187\pm427.428$ & $0.899\pm0.251$ & $50.506$\\
LOMMA+KEDMI & $0.593\pm0.012$ & $0.770\pm0.011$ & $1806.098\pm528.101$ & $0.782\pm0.305$ & $54.407$\\
\bottomrule
    \end{tabular}
    }
    \end{threeparttable}
    % \vspace{-1em}
\end{table}

==> tables/ffhq64_facescrub64_ir152_low/prdc.tex <==
\begin{table}[!ht]
    \setlength{\tabcolsep}{5pt}
    \normalsize
    \centering
    \caption{\todo{table}}
    \label{}
    \begin{threeparttable} 
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccccc}
        \toprule
\textbf{Method} & $\uparrow\textbf{Precision}$ & $\uparrow\textbf{Recall}$ & $\uparrow\textbf{Density}$ & $\uparrow\textbf{Coverage}$\\ \midrule
GMI & $0.057\pm0.113$ & $\mathbf{0.868}\pm0.143$ & $0.015\pm0.035$ & $0.038\pm0.070$\\
KEDMI & $0.067\pm0.184$ & $0.020\pm0.110$ & $0.019\pm0.047$ & $0.027\pm0.054$\\
Mirror & $\mathbf{0.209}\pm0.239$ & $0.422\pm0.293$ & $\mathbf{0.067}\pm0.084$ & $\mathbf{0.136}\pm0.134$\\
PPA & $0.124\pm0.177$ & $0.531\pm0.270$ & $0.035\pm0.056$ & $0.077\pm0.097$\\
PLGMI & $0.047\pm0.114$ & $0.330\pm0.295$ & $0.015\pm0.026$ & $0.033\pm0.057$\\
LOMMA+GMI & $0.074\pm0.131$ & $0.653\pm0.258$ & $0.024\pm0.048$ & $0.050\pm0.077$\\
LOMMA+KEDMI & $0.065\pm0.179$ & $0.006\pm0.067$ & $0.022\pm0.044$ & $0.028\pm0.049$\\
\bottomrule
    \end{tabular}
    }
    \end{threeparttable}
    % \vspace{-1em}
\end{table}

==> tables/ffhq64_facescrub64_ir152_mid/base.tex <==
\begin{table}[!ht]
    \setlength{\tabcolsep}{5pt}
    \normalsize
    \centering
    \caption{\todo{table}}
    \label{}
    \begin{threeparttable} 
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccccc}
        \toprule
\textbf{Method} & $\uparrow{\mathbf{Acc}@1}$ & $\uparrow{\mathbf{Acc}@5}$ & $\downarrow\mathbf{\delta}_{eval}$ & $\downarrow\mathbf{\delta}_{face}$ & $\downarrow\textbf{FID}$\\ \midrule
GMI & $0.223\pm0.113$ & $0.368\pm0.127$ & $2374.313\pm310.858$ & $1.130\pm0.191$ & $94.172$\\
KEDMI & $0.434\pm0.013$ & $0.620\pm0.016$ & $2124.271\pm587.946$ & $0.963\pm0.346$ & $89.364$\\
Mirror & $0.462\pm0.028$ & $0.626\pm0.024$ & $1812.977\pm440.571$ & $0.912\pm0.277$ & $32.502$\\
PPA & $0.829\pm0.039$ & $0.902\pm0.028$ & $1413.097\pm468.792$ & $0.683\pm0.240$ & $\mathbf{30.618}$\\
PLGMI & $\mathbf{0.965}\pm0.005$ & $\mathbf{0.981}\pm0.004$ & $\mathbf{1163.656}\pm362.421$ & $\mathbf{0.557}\pm0.153$ & $78.283$\\
LOMMA+GMI & $0.517\pm0.119$ & $0.670\pm0.104$ & $2071.116\pm381.253$ & $0.894\pm0.206$ & $71.598$\\
LOMMA+KEDMI & $0.654\pm0.006$ & $0.823\pm0.007$ & $1771.850\pm504.995$ & $0.734\pm0.272$ & $69.925$\\
\bottomrule
    \end{tabular}
    }
    \end{threeparttable}
    % \vspace{-1em}
\end{table}

==> tables/ffhq64_facescrub64_ir152_mid/prdc.tex <==
\begin{table}[!ht]
    \setlength{\tabcolsep}{5pt}
    \normalsize
    \centering
    \caption{\todo{table}}
    \label{}
    \begin{threeparttable} 
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccccc}
        \toprule
\textbf{Method} & $\uparrow\textbf{Precision}$ & $\uparrow\textbf{Recall}$ & $\uparrow\textbf{Density}$ & $\uparrow\textbf{Coverage}$\\ \midrule
GMI & $0.030\pm0.076$ & $\mathbf{0.865}\pm0.161$ & $0.009\pm0.022$ & $0.023\pm0.047$\\
KEDMI & $0.038\pm0.125$ & $0.037\pm0.155$ & $0.010\pm0.031$ & $0.016\pm0.038$\\
Mirror & $\mathbf{0.220}\pm0.231$ & $0.462\pm0.296$ & $\mathbf{0.073}\pm0.093$ & $\mathbf{0.145}\pm0.147$\\
PPA & $0.128\pm0.183$ & $0.514\pm0.286$ & $0.039\pm0.066$ & $0.083\pm0.107$\\
PLGMI & $0.040\pm0.105$ & $0.319\pm0.301$ & $0.013\pm0.025$ & $0.027\pm0.050$\\
LOMMA+GMI & $0.040\pm0.100$ & $0.632\pm0.262$ & $0.011\pm0.022$ & $0.025\pm0.041$\\
LOMMA+KEDMI & $0.041\pm0.157$ & $0.000\pm0.000$ & $0.011\pm0.032$ & $0.013\pm0.039$\\
\bottomrule
    \end{tabular}
    }
    \end{threeparttable}
    % \vspace{-1em}
\end{table}

==> tables/ffhq64_facescrub64_vgg16/prdc.tex <==
\begin{table}[!ht]
    \setlength{\tabcolsep}{5pt}
    \normalsize
    \centering
    \caption{\todo{table}}
    \label{}
    \begin{threeparttable} 
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccccc}
        \toprule
\textbf{Method} & $\uparrow\textbf{Precision}$ & $\uparrow\textbf{Recall}$ & $\uparrow\textbf{Density}$ & $\uparrow\textbf{Coverage}$\\ \midrule
GMI & $0.050\pm0.109$ & $\mathbf{0.778}\pm0.176$ & $0.017\pm0.032$ & $0.040\pm0.076$\\
KEDMI & $0.047\pm0.118$ & $0.113\pm0.230$ & $0.014\pm0.047$ & $0.026\pm0.072$\\
Mirror & $\mathbf{0.187}\pm0.221$ & $0.459\pm0.296$ & $\mathbf{0.070}\pm0.100$ & $\mathbf{0.137}\pm0.147$\\
PPA & $0.118\pm0.176$ & $0.517\pm0.281$ & $0.041\pm0.074$ & $0.087\pm0.118$\\
PLGMI & $0.047\pm0.124$ & $0.099\pm0.194$ & $0.016\pm0.061$ & $0.026\pm0.077$\\
LOMMA+GMI & $0.069\pm0.136$ & $0.560\pm0.277$ & $0.021\pm0.050$ & $0.043\pm0.077$\\
LOMMA+KEDMI & $0.061\pm0.198$ & $0.000\pm0.000$ & $0.020\pm0.066$ & $0.020\pm0.052$\\
\bottomrule
    \end{tabular}
    }
    \end{threeparttable}
    % \vspace{-1em}
\end{table}


==> tables/metfaces256_celeba224_resnet152/prdc.tex <==
\begin{table}[!ht]
    \setlength{\tabcolsep}{5pt}
    \normalsize
    \centering
    \caption{\todo{table}}
    \label{}
    \begin{threeparttable} 
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccccc}
        \toprule
\textbf{Method} & $\uparrow\textbf{Precision}$ & $\uparrow\textbf{Recall}$ & $\uparrow\textbf{Density}$ & $\uparrow\textbf{Coverage}$\\ \midrule
GMI & $0.003\pm0.024$ & $0.447\pm0.379$ & $0.001\pm0.004$ & $0.002\pm0.010$\\
KEDMI & $0.002\pm0.025$ & $0.000\pm0.005$ & $0.001\pm0.004$ & $0.001\pm0.005$\\
Mirror & $\mathbf{0.163}\pm0.230$ & $0.272\pm0.303$ & $\mathbf{0.038}\pm0.050$ & $\mathbf{0.073}\pm0.083$\\
PPA & $0.157\pm0.226$ & $0.250\pm0.292$ & $0.036\pm0.047$ & $0.068\pm0.080$\\
PLGMI & $0.000\pm0.000$ & $0.000\pm0.000$ & $0.000\pm0.000$ & $0.000\pm0.000$\\
LOMMA+GMI & $0.000\pm0.009$ & $\mathbf{0.615}\pm0.422$ & $0.000\pm0.004$ & $0.001\pm0.005$\\
LOMMA+KEDMI & $0.000\pm0.000$ & $0.001\pm0.016$ & $0.000\pm0.002$ & $0.000\pm0.003$\\
\bottomrule
    \end{tabular}
    }
    \end{threeparttable}
    % \vspace{-1em}
\end{table}

==> tables/metfaces256_facescrub224_resnet152/base.tex <==
\begin{table}[!ht]
    \setlength{\tabcolsep}{5pt}
    \normalsize
    \centering
    \caption{\todo{table}}
    \label{}
    \begin{threeparttable} 
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccccc}
        \toprule
\textbf{Method} & $\uparrow{\mathbf{Acc}@1}$ & $\uparrow{\mathbf{Acc}@5}$ & $\downarrow\mathbf{\delta}_{eval}$ & $\downarrow\mathbf{\delta}_{face}$ & $\downarrow\textbf{FID}$\\ \midrule
GMI & $0.032\pm0.004$ & $0.101\pm0.017$ & $\mathbf{110.653}\pm23.770$ & $1.377\pm0.167$ & $153.889$\\
KEDMI & $0.012\pm0.001$ & $0.038\pm0.006$ & $148.593\pm42.485$ & $1.566\pm0.239$ & $317.361$\\
Mirror & $0.117\pm0.006$ & $0.293\pm0.016$ & $241.134\pm38.587$ & $1.314\pm0.211$ & $66.567$\\
PPA & $0.471\pm0.036$ & $0.738\pm0.036$ & $201.933\pm35.690$ & $1.132\pm0.207$ & $\mathbf{63.775}$\\
PLGMI & $\mathbf{0.801}\pm0.010$ & $\mathbf{0.954}\pm0.004$ & $134.861\pm37.059$ & $\mathbf{0.866}\pm0.201$ & $165.756$\\
LOMMA+GMI & $0.131\pm0.039$ & $0.285\pm0.057$ & $114.550\pm35.304$ & $1.293\pm0.218$ & $190.903$\\
LOMMA+KEDMI & $0.008\pm0.001$ & $0.023\pm0.002$ & $203.183\pm76.346$ & $1.678\pm0.236$ & $368.632$\\
\bottomrule
    \end{tabular}
    }
    \end{threeparttable}
    % \vspace{-1em}
\end{table}

==> tables/metfaces256_facescrub224_resnet152/prdc.tex <==
\begin{table}[!ht]
    \setlength{\tabcolsep}{5pt}
    \normalsize
    \centering
    \caption{\todo{table}}
    \label{}
    \begin{threeparttable} 
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccccc}
        \toprule
\textbf{Method} & $\uparrow\textbf{Precision}$ & $\uparrow\textbf{Recall}$ & $\uparrow\textbf{Density}$ & $\uparrow\textbf{Coverage}$\\ \midrule
GMI & $0.018\pm0.063$ & $0.329\pm0.342$ & $0.004\pm0.010$ & $0.008\pm0.021$\\
KEDMI & $0.003\pm0.048$ & $0.016\pm0.096$ & $0.000\pm0.003$ & $0.000\pm0.003$\\
Mirror & $\mathbf{0.192}\pm0.236$ & $0.339\pm0.322$ & $\mathbf{0.042}\pm0.054$ & $\mathbf{0.080}\pm0.093$\\
PPA & $0.171\pm0.223$ & $0.303\pm0.309$ & $0.042\pm0.062$ & $0.075\pm0.095$\\
PLGMI & $0.007\pm0.062$ & $0.000\pm0.000$ & $0.003\pm0.014$ & $0.003\pm0.012$\\
LOMMA+GMI & $0.008\pm0.052$ & $\mathbf{0.409}\pm0.421$ & $0.001\pm0.006$ & $0.003\pm0.011$\\
LOMMA+KEDMI & $0.001\pm0.026$ & $0.018\pm0.115$ & $0.000\pm0.003$ & $0.000\pm0.002$\\
\bottomrule
    \end{tabular}
    }
    \end{threeparttable}
    % \vspace{-1em}
\end{table}
